CASS: Towards Building a Social-Support Chatbot for Online Health Community

Chatbots systems, despite their popularity in today's HCI and CSCW research, fall short for one of the two reasons: 1) many of the systems use a rule-based dialog flow, thus they can only respond to a limited number of pre-defined inputs with pre-scripted responses; or 2) they are designed with a focus on single-user scenarios, thus it is unclear how these systems may affect other users or the community. In this paper, we develop a generalizable chatbot architecture (CASS) to provide social support for community members in an online health community. The CASS architecture is based on advanced neural network algorithms, thus it can handle new inputs from users and generate a variety of responses to them. CASS is also generalizable as it can be easily migrate to other online communities. With a follow-up field experiment, CASS is proven useful in supporting individual members who seek emotional support. Our work also contributes to fill the research gap on how a chatbot may influence the whole community's engagement.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> old copies/1_introduction.tex <==

\section{INTRODUCTION}


Women are at \pzh{a} high risk of mental illness during pregnancy and within one year of delivery          \cite{Ishibe2006Incidence}. 
% In developing and developed countries, the incidence of having perinatal depression is 5\%-30\% and 20\% respectively         \cite{Pereira2009Depression}. 
% naturalistic,
For example, in a  longitudinal study with over 1000 pregnant women, Banti et al. found that 12.4\% of them suffer from depression in pregnancy, and 9.6\% of them encounter depression in the postpartum period          \cite{Banti2011From}.
% The prevalence of depression in pregnancy was 12.4\%, and the probability of postpartum depression was 9.6\%         \cite{Banti2011From}. 
% Moreover, depression in pregnant women may impact the brain development pattern of infants          \cite{rifkingraboi2013prenatal}.
The rapidly emerging online health communities (OHCs) offer an accessible place for pregnant women to exchange social support about their depressing issues           \cite{social_support_article}.  
% Nowadays, online health communities are emerging rapidly, which provides people with a place to seek and exchange social support          \cite{social_support_article}. 
They share advice, informal and
formal knowledge and emotional support from peers during each stage of pregnancy          \cite{Pregnant_community_Gui:2017:ISS:3171581.3134685,Wierckx:2014:BAS:2559206.2581179,drentea2005social}. 
% Many of which are specifically for pregnant women         \cite{Pregnant_community_Gui:2017:ISS:3171581.3134685,Wierckx:2014:BAS:2559206.2581179,drentea2005social}.

The OHCs are generally considered beneficial to the members inside, such as inducing positive cognitive change          \cite{moment_of_change_Pruksachatkun:2019:MCA:3290605.3300294} and enhancing social connectiveness          \cite{peer-to-peer-support-risks-benefits}. 
However, many of the help-seeking posts in OHCs can not get replies from others          \cite{no_reply_community:article}. 
% However, there are still some problems in the community. 
% The commitment of the community has been proved to be significantly affected by emotional support         \cite{To_stay_or_leave_Wang:2012:SLR:2145204.2145329}. 
% Many of the help-seeking posts (e.g., 10\% posts in the communities reported in          \cite{no_reply_community:article}) in OHCs could not get replies. 
The lack of timely response could discourage the help-seekers, resulting in their withdrawal from OHCs and further isolation          \cite{Design_Opportunities_for_Mental_Health_Peer_Support_TechnologiesO'Leary:2017:DOM:2998181.2998349}. 
Also, it could impair the development of the OHCs with a likely reduction of members' commitment          \cite{To_stay_or_leave_Wang:2012:SLR:2145204.2145329}. 
% If they get a lot of support and emotional support, members are more likely to stay, and the community will be more durable         \cite{To_stay_or_leave_Wang:2012:SLR:2145204.2145329}. 

Recent advance of the chatbots \pzh{offers} an opportunity for OHCs to address the problem of low response rate by automatically generating replies to the posts. 
% Deploying a chatbot in the community which can provide timely emotional support may help to address these problems. 
Chatbots have been widely used in various fields,  
\pzh{acting as customer service agents          \cite{chatbot_service_agent_Xu:2017:NCC:3025453.3025496, customer_engagement_tone}, human assistant          \cite{AllWork:Liao:2018:WNP:3173574.3173577}, and healthcare givers          \cite{inproceedings}.}
% such as acting as an agent to answer customer inquiries         \cite{chatbot_service_agent_Xu:2017:NCC:3025453.3025496, customer_engagement_tone}, serving as a human assistant         \cite{AllWork:Liao:2018:WNP:3173574.3173577}, and involving with health-related domains         \cite{inproceedings}.
Previous work has attempted to discuss the deployment of chatbots to communities          \cite{Recommend_comment_Morris2018TowardsAA,Community_member:Seering:2019:BDI:3290605.3300680}. 
However, these works in health domains \pzh{mostly focus on the chatbot's one-on-one interaction with human but mostly overlook its influence on the communities}. 
Questions raise on how would the chatbot work as a member in OHCs and how would its automatic response affect the behaviors of help-seekers and other members. 

% Few works allow chatbots to interact with others in the community as a completely independent member and analyze the impact of chatbot on the community. Chatbot technology is developing day by day, such as rule-based         \cite{ASurveyOnDialogueSystemChen:2017:SDS:3166054.3166058}, retrieval-based         \cite{Retrieval1:Yan:2016:LRD:2911451.2911542} and generation-based         \cite{Generation1:Serban:2016:BED:3016387.3016435}. Advanced deep learning technologies, such as long short-term memory(LSTM) networks, are applied to customer service on social media         \cite{chatbot_service_agent_Xu:2017:NCC:3025453.3025496}. This makes it possible for us to create a chatbot to provide emotional support to pregnant women that did not get a response to their post in the online community.

As an initial probe to address the questions above, we build up the chatbot, which is framed as a human member and automatically leaves replies to the pregnant women in OHCs. 
Specifically, we use the well-developed LSTM (Long Short-Term Memory) network to train our chatbot in a large dataset collected from an OHC for pregnant women care. 
After verifying the appropriateness of the contents generated by chatbot offline, we deploy it to the same OHC for pregnant women care for a seven-days between-subjects field study. 
The results show that chatbot's replies improve the overall reply speed of posts. Hosts (i.e., the help-seekers) are more active in replying to others. In replying others' replies, hosts are willing to communicate more about their thoughts and disclose more about their situation. Furthermore, chatbot's replies stimulate more emotion raise and less emotion drop of the hosts. 
% We expect to use advanced deep learning technology to create a chatbot for pregnant women and interact with other members in a one-to-many manner as a member of the community. However, there was no work to provide emotional support to pregnant women in the community with the anonymous chatbot. We hope that through our field study, we can explore whether this method is reasonable, whether it can have a positive effect on individuals and communities, and whether it may have adverse consequences. We expect our chatbot to bring emotional support to pregnant women. Moreover, it can have a positive impact on community dynamics.



% We trained an emotional support chatbot(chatbot:\textbf{Emo}tional \textbf{s}upport \textbf{Bot}) for pregnant women through LSTM network based on an online pregnant women's community, using public data from the community as a corpus. Moreover, we deployed chatbot to the online pregnant community and conducted a seven-days between-subjects field study. We found that chatbot’s replies improve the overall reply speed of posts. Hosts are more active in replying to others. In replies host replied to the chatbot, hosts are willing to express more communication and emotion disclosure. Furthermore, chatbot's replies inspire host more emotion raise and less emotion drop. 

The main contributions of our work are:
\begin{itemize}
    \item We built chatbot which can reply timely to the help-seekers in OHCs for pregnant women.
    \item We deployed chatbot to a real online pregnant women's community and conducted a seven-days between-subjects study to analyze the impact on community building and individuals' well-being. And we found replies of chatbot improve the overall reply speed of posts. Hosts are more active in replying to others, \pzh{and they reply to the chatbot with emotional disclosure and more emotion raise.}
    % and replying to a chatbot with emotional disclosure and more emotion raise. 
    \item We discussed the interaction between the chatbot and members in OHCs and examined which type of replies can attract others and the superiority of chatbot.
\end{itemize}



% 1. pregnant women's emotional need and response rate and time problem

% 2. CA is popular

% 3. CA support community, health related
  
% 4. CA for healthcare community:there is some work but not deploy in community and examine how did chatbot affect the community.
% %these  chatbots  are  for  one-on-one  care. There is a gap on understanding how would a chat-bot member for providing (emotional) support work in health community         \cite{Community_member:Seering:2019:BDI:3290605.3300680}         \cite{Recommend_comment_Morris2018TowardsAA}

% 6. Recent advances in AI and NLP show that chatbots can probably serve as supportive members in those communities

% 7. RQ: A Study on the Impact of Bot as an Active Member of healthcare Community

% 8.challenges:Proposed by Zhenhui

% 8.what we did

% 9.contribution

%     a.bot for pregnant women
    
%     b.the effect study
    
%     c.Give some advice or guidelines




\iffalse
1. The conversational agent is getting popularized among every aspect in the society, it provides convenience to people to seek information, while in the meantime saving efforts for the service providers. Although it has widely been used, we have not get a feedback for users that have used it.

2. Online community has been facing challenges, such as keeping the posts active, 

3. We choose to do the pilot study on a pregnancy community because it is a special stage of life where nearly every family has to been through. These expectant mother share common characteristics, such as perinatal depression, and encountering health problems before and after giving birth, etc. This community gathers people of similar stage in life. Therefore we study.

4. New generative model technologies expose new possibilities

5. So our topic/theme for this study is...

\zhenhui{Notes by Zhenhui, based on 8/8 meetings (Citation needed)
\begin{itemize}
    \item General background
    \begin{itemize}
        \item Online health communities are popular.
        \item The common interactions in these communities, like exchange of informational and emotional support.
        \item They are effective, but have several challenges (we can choose one or more):
        \begin{itemize}
            \item Low response rate
            \item Support are not timely
            \item Some comments are unsupportive
        \end{itemize}
    \end{itemize}
    \item General motivation
    \begin{itemize}
        \item There are some researches show that a supportive response can induce other members to provide help to the support seekers. (One paper: What to Say to an Online Support-Seeker? The Influence of Others' Responses and Support-Seekers' Replies)
        \item However, a person that can always give timely support is hard to find. 
        \item Recent advances in AI and NLP show that chatbots can probably serve as supportive members in those communities. 
        \item Chatbots are popular, serving people in various contexts.
        \item In the domains of health care, some researchers have explore the roles of chatbots as health providers or receivers. 
        \item These works show that chatbots are effective in health care. 
        \item However, these chatbots are for one-on-one care. There is a gap on understanding how would a chatbot member for providing (emotional) support work in health community (May need to specify pregnant community in the background?).
    \end{itemize}
    \item Challenges
    \begin{itemize}
        \item Applying chatbots as members in the health care communities are challenging.
        \item 1. Can the responses from AI chatbots be appropriate and supportive (to the specific post)? (Could match to the current rating results and further rating results after deployment) There are many examples in which chatbot responses are not good as human responses. This is about whether the technology is enough and what needs further development.
        \item 2. Would the community members accept and trust chatbot? Human-AI relationship issues. People with health issues may have difficulties interacting with AI chatbots, e.g., they may be sensitive of being judged by algorithms (a CHI 2019 paper); they prefer efforts from human peers (emphatic chatbot paper).
    \end{itemize}
    \item Proposed Work
    \begin{itemize}
        \item Build up an AI chatbot
        \item Deploy in a pregnant health community for a week.
        \item Compare the posts with/without chatbot.
        \item Check how chatbot affect community dynamics and how members interact with chatbot.
        \item ...
    \end{itemize}
    \item Contributions
    \begin{itemize}
        \item 
    \end{itemize}
\end{itemize}
% My concern here is: should we let users know that this is a chatbot during interaction or pretend chatbot as a human member? It may be related to ethic issues and whether we can put it into the normal human-agent interaction contexts about acceptance and trust (usually they know they are interacting with AIs).

%{Throughout the interaction cycle, our AI active in the community as a human member. After data collection is completed, we will expose our identity to users. For ethical issues, we have done the following measures: filtering hit words, real-time monitoring of users interacting with AI, and timely explanation to users at the end of the experiment.}
}

\fi

==> old copies/2_related_work.tex <==

\section{Related Work}
% Current flow based on the general research question (my YY...): 

% \textbf{How would a chatbot that automatically provides emotional support affects the dynamics of a pregnant women online community?}

\subsection{Engaging Members in Online Health Community}
Existing OHCs have experimented a variety of ways to engage their members in active discussion and sharing             \cite{build_successful_community:Kraut:2012:BSO:2207798}. 
% (The work by Preece suggested the social determinants for success of online communities can be measured on the number of messages per unit of time, amount of interactivity (thread depth), reciprocity (taking from and giving back to the community), and so on             \cite{build_successful_community:Kraut:2012:BSO:2207798}) (Not match to the context). 
From the aspects of members who create the posts, works have been done to identify what kinds of post can attract more responses. 
For example, in the communities that discuss topics ranging from technical support to health, Arguello et. al found that posting on-topic, introducing oneself via autobiographical testimonials, asking questions, using less complex language and other features of the messages, increased replies             \cite{talk_to_me:Arguello:2006:TMF:1124772.1124916}. 
Communities like Reddit r/depression \footnote{https://www.reddit.com/r/depression/} offer guidelines to the posters to help them express their needs more explicitly to get replies. 
Also, some communities, such as YOUBAOBAO, provides features like profile information and photo with faces, which could help attract more ``likes'' and comments             \cite{face_attract_Bakhshi:2014:FEU:2556288.2557403}. 
From the aspects of people who leave comments under others' posts, many OHCs like those on Reddit (e.g., r/pregnant \footnote{https://www.reddit.com/r/pregnant/}) apply reward structures, such as the upvoting and downvoting. 
These rewarding systems could stimulate them to reply others' posts in a good manner.
However, given the large amount of posts in the community, these approaches mentioned above could not ensure that all posts, especially those which explicitly seek support, get timely replies. 

Building an automatic chatbot to offer support to these posts could be a promising way to address the posters' need and improve the others' attention to engage in the posts. 
Li et. al suggested that a supportive comment under one's post can induce other members to join and provide supportive comments to the post             \cite{support_others_doi:10.1111/hcre.12055}. 
We are interested to check whether a chatbot can act as such a supportive member that provides the first emotional support, and how would such a chatbot affect the dynamic of the community engagement on this post.

% \begin{itemize}
%     \item From the aspects of people who create posts
%     \begin{itemize}
%         \item post ranking -- the recommendation system
%         \item post content -- on-topic, introducing oneself via autobiographical testimonials, asking questions, using less complex language and other features of the messages, increased replies.  Talk to Me: Foundations for Successful Individual-Group Interactions in Online Communities (CHI 2006)   Norms Matter: Contrasting Social Support Around Behavior Change in Online Weight Loss Communities (CHI 2018)   How Collaborative Editing with Mentors Improves Engagement in Social Q\&A Communities (CHI 2018)
%         \item ...
%         \item Potential drawback -- in online health communities
%     \end{itemize}
%     \item From the aspects of people who leave comments
%     \begin{itemize}
%         \item Gamification elements -- Personalizing Persuasive Strategies in Gameful Systems to Gamification User Types (CHI 2017), reward, social comparison, e.g., (upvoting, downvoting, reputation system in Reddit)
%         \item Face photo -- Faces engage us: photos with faces attract more likes and comments on Instagram (CHI 2014)
%         \item ...
%         \item potential drawback -- in online health communities, xxx --> many posts still can not get response.
%         \item A promising yet unexplored way is use chatbot to simulate a community member             \cite{Community_member:Seering:2019:BDI:3290605.3300680}
%         \item A work show that a member with supportive comment can induce others to join and provide supportive comments to others. ``What to Say to an Online Support-Seeker? The Influence of Others' Responses and Support-Seekers' Replies''
%     \end{itemize}
%     \item In this paper, we explore the effectiveness of using a chatbot as a member to automatically provide support, checking whether and how it would affect the members' engagement in the community. 
% \end{itemize}

% Importance and benefit of (emotional) support in such community for pregnancy.

% Our work aims in ...




\subsection{Emotional Support in Online Health Community}
% \begin{itemize}
%     \item General description of online health community,  social support: informational + emotional
%     \item The benefit of the online health community.
%     \item The drawback in such community, especially the cases that many posts can not get timely responses and some comments lack emotional support that is important.
%     \item The case of pregnant woman online community.
%     \item Argument for our choice on the community and research question (e.g., why emotional support).
% \end{itemize}
% Women during pregnancy or within one year of giving birth can easily encounter depressing moments             \cite{depression_pregnancy:Barry:2017:MMM:3025453.3025918, pregnancy_depressionarticle}. 
% For example, a report in 

Online health communities (OHCs) offer an accessible place for people who have a common concern to seek and exchange social support             \cite{social_support_article}. 
Researches on these communities have looked into what types of support are shared             \cite{To_stay_or_leave_Wang:2012:SLR:2145204.2145329}, how support is different across platforms and communities             \cite{linguisticSharma:2018:MHS:3173574.3174215},  social roles of the members             \cite{seekers:Yang:2019:SPW:3290605.3300574}, and the effects of channels on self disclosure             \cite{Channel:Yang:2019:CMS:3290605.3300261}. 
Among different types of social support, emotional support (i.e., the understanding,
encouragement, affirmation, sympathy, or caring towards the help seekers             \cite{To_stay_or_leave_Wang:2012:SLR:2145204.2145329, Social_support_definition:Bambina:2007:OSS:1534606}) is  identified as the common and effective support in online health communities             \cite{Emotional_support_UdenKraan2012BreastC}. 

% (Sorry, the logic of this part is still a mess...)
% ``Engagement with Mental Health Screening on Mobile Devices: Results from an Antenatal Feasibility Study'' (CHI 2019) 
% (Abstract) Perinatal depression (PND) affects up to 15\% of women within the United Kingdom and has a lasting impact on a woman's quality of life, birth outcomes and her child's development.


As for the OHCs specifically for pregnant women, Gui et al. found that pregnant women consistently sought advice, informal and formal knowledge, reassurance, and emotional support from peers during each stage of pregnancy             \cite{Pregnant_community_Gui:2017:ISS:3171581.3134685}. 
They found that 9.5\%, 10.0\% and 12.0\% of the posts are related to emotional stress in early, middle and late pregnancy stage, respectively. 
These posts are about miscarriage, changes to their life, fear about upcoming birth and extreme physical discomfort. 
Fourney et al. identified that people use words about emotional states (e.g., worried, terrified, scared) to search about pregnancy and childbirth, which express their emotional concerns             \cite{Search_pregnancyFourney:2015:ETC:2702123.2702427}. 
In fact, women could easily encounter depressed moments during pregnancy             \cite{depression_pregnancy:Barry:2017:MMM:3025453.3025918, pregnancy_depressionarticle}. 
It is thus necessary for the OHCs to provide timely emotional support to the pregnant women, especially to those who explicitly seek it in the community. 
However, many of the help-seeking posts (e.g., 10\% posts in the communities reported in             \cite{no_reply_community:article}) in OHCs could not get replies. 
% For example,  have no replies. 
This could not only do harm to the pregnant women in depressing status             \cite{Depressed_women_Leigh2008RiskFF}, but also impair the long-term development of the OHCs             \cite{build_successful_community:Kraut:2012:BSO:2207798}. 


% In this work, we seek to design simulate a peer with an automatic chatbot to provide emotional support to the posters in online pregnant women community. 




\subsection{Chatbots in Health Domains and in Online Community}
% \begin{itemize}
%     \item The very first case of chatbot, ELIZA, simulating a therapist.
%     \item Popular in various topics.
%     \item Recent trend about their applications in health domains, e.g., WeoBot, Bot for ...  
%     \item Mostly one on one separately, few cases in community (if any, discuss them)
%     \item How could such a chatbot affect the community dynamic and be perceived by members, are under investigated. 
% \end{itemize}

Since the first role as a psychotherapist in 1960s             \cite{ELIZA:Weizenbaum:1966:ECP:365153.365168}, chatbots have been taking a variety of social roles to converse with human naturally             \cite{Chatterbot:Mauldin:1994:CTT:199288.199285}. 
For example, chatbots can serve as agents to answer customers' requests             \cite{chatbot_service_agent_Xu:2017:NCC:3025453.3025496, customer_engagement_tone}, or group chat facilitators that assign tasks             \cite{TaskManagement:Toxtli:2018:UCT:3173574.3173632} and summarize information             \cite{MakeSenseGroupChat:Zhang:2018:MSG:3290265.3274465}, or act as human resource assistants to interact with new hires             \cite{AllWork:Liao:2018:WNP:3173574.3173577}. 
% (Need better transition here.)
The widely accessible chatbots also attract eyes in the health-related domains. 
For instance, Fitzpatrick et al. deployed Woebot to deliver web-based cognitive behavior therapy to young adults and found that it can reduce their depression             \cite{woebot}. 
Lee et al. designed Vincent, a chatbot that is showed to improve user self-compassion through exchange of care             \cite{self-compassion}. 
Schroeder et al. embedded a conversational agent into a mobile app to support dialectical behavioral therapy and their participants reported decreased anxiety after the weeks-long field study             \cite{DBT:Schroeder:2018:PSC:3173574.3173972}. 
Despite the effectiveness of chatbots in the one-on-one health care, It is unclear what will be their influences when applied in online health communities. 

% \textcolor{red}{twitter bot?}

Deploying chatbots in online communities is not new and there are a lot of works to analyze the effects of these bots. 
For example,  Gilani et al. found that the bots in Twitter play a significant role in boosting the popularity of post content             \cite{TwitterBotGilani:2017:BIT:3041021.3054255}. 
Similarly, Johnson et al. analyzed content
about United States and China in Wikipedia and found that automatic content generation by bots is critical for ensuring that there is any content at all about some rural areas             \cite{Wikipedia:Johnson:2016:HRP:2858036.2858123}. 
Peng et al. found that the chatbot which recommends reviewers for pull requests in GitHub can reduce the response time of first comment by any developer             \cite{Peng2019}. 
In a work that is more closed to health domains, Morris et al. used information retrieval techniques to build up an empathic conversational agent and deployed it in a mental health community             \cite{Recommend_comment_Morris2018TowardsAA}. 
Their studies revealed that 79.8\% responses from the agent were deemed acceptable by users, but users preferred the efforts of their peers more than those from the agent. 
However, they did not examine how did the chatbot affect the community dynamics. 
In fact, according to the review in             \cite{Community_member:Seering:2019:BDI:3290605.3300680}, few works have explored chatbots as community members. 
% (Should need other words to emphasize the importance. Or discuss it in next part?)
Therefore, our work looks into framing the chatbot as a community member and check how would it affect the online health community. 


% \zhenhui{
% \subsection{Engaging Members in Online Community}
% Note: what do you think should be the theme of the third-part of related work.

% Note by liuping: A lot of research has focused on how to build a sustainable and successful community. We are trying to add such an automated robot to activate the community and increase the participation of other members.


% }

% \subsection{Generative Dialogue Model}
% note by liuping: maybe we should add this part. New generative model technologies expose new possibilities. Discuss the development of some generation models of Chatbot. We are characterized by the use of pregnant women-related corpus in specific areas of pregnant women. More specific and unique. 
% \zhenhui{Noted by Zhenhui: I think we do not need to add this part. This is not our focus, the chatbot is served as one solution to address the lack-of-response problem. In fact, there are a lot of chatbot solutions. The chatbot we developed is likely not the best. We need to give a convincing argument of why we use these techniques to build such a chatbot, at the beginning of design section.}

% \subsection{Chatbots in Online Communities}
% There are some works that focus on developing or analyzing the chatbots in online communities. 


==> old copies/3_system.tex <==
\section{The Experimental Chatbot}
% \color{red}
% \begin{itemize}
%     \item overall intro
%     \item classification model
%     \begin{itemize}
%         \item method
%     \end{itemize}
%     \item generate model
%     \begin{itemize}
%         \item method
%     \end{itemize}
%     \item implementation
%     \item Performance
%     \begin{itemize}
%         \item auto
%         \item human
%     \end{itemize}
% \end{itemize}
% \color{black}



Before describing the study, we would like to introduce the auto-reply chatbot. The chatbot is composed of two parts: the classification model and the reply generation model.

\begin{itemize}
    \item Classification model: According to the text content of a post, chatbot identifies the type of post as one of emotional seeking and informational seeking.
    \item Reply generation model: Based on the text content of the post, chatbot automatically generates a reply using deep learning algorithm.
\end{itemize}


\subsection{Classification Model}
As suggested by previous work    \cite{To_stay_or_leave_Wang:2012:SLR:2145204.2145329}, two types of the categories of social support which have received the most theoretical and empirical attention are emotional support and informational support. To avoid involving professional medical issues, we build emotion-seeking/information-seeking posts classification model to filter out information-seeking posts.

Convolutional Neural network(CNN) model has been widely used in the computer vision field    \cite{Krizhevsky2012ImageNet} in these years, and has also been extended to the field of text classification     \cite{kim2014convolutional}. CNN model is proposed in this work for classifying post type. We embed the posts to word vector, which is 64 dimensions, and then we fed these vectors into the CNN model. Specifically, the input layer of the CNN model in our system has 600 neurons, and the total CNN uses a simple structure, including one convolutional layer and two full-connection layers. The convolutional layer consists of three consecutive operations: convolution with kernels, non-linear activation function, and max pooling. The convolutional layer contains 256 kernels, and the FC layer contains 128 units with a dropout rate of 0.5. We optimized the model with AdamOptimizer using a learning rate of 0.001. After training the model, we conducted 5-fold cross-validation. 

\subsection{Reply Generation Model}
The conversation between users and the chatbot can be regarded as input a sequence of words representing the post and outputting a sequence of words representing the reply according to the input sequence. 

In our system, we used OpenNMT    \cite{Klein2018OpenNMT}, which is a state-of-the-art open-source toolkit\footnote{https://opennmt.net/} for neural machine translation (NMT), to build a model to generate reply according to a post. The model was based initially on sequence-to-sequence with attention mechanism     \cite{Luong2015Effective}. The source words are first mapped to word vectors and then fed into a Long Short-Term Memory network(LSTM)    \cite{HochreiterLong}. Upon seeing the heosi symbol, the final time step initializes a target orange LSTM. At each target time step, attention is applied over the source LSTM and combined with the current hidden state to produce a prediction of the next word. This prediction is then fed back into the target LSTM. Specifically, we trained these deep LSTMs jointly with two layers * 500 memory cells using stochastic gradient descent and 0.2 dropout. The batch size is 64, and the global attention translation is mlp. We trained 100000 steps to fit it.


% \begin{figure}
% \centering
%   \includegraphics[width=0.9\columnwidth]{figures/seq2seq.png}
%   \caption{Sequence-to-sequence learning with LSTM neural networks}~\label{fig:lstm}
% \end{figure}



\subsection{Implementation}
We collected 220,000 post-reply pairs from the online community\footnote{http://youbaobao.meiyou.com/}. All data we obtained are public and made available from the community via their application programming interface (API). Specifically, this does not include any data that has been marked as 'private' by the author or any direct messages. 


\textit{Classification Model}.
We randomly select one-month data for labeling procedure. %Firstly, Two authors label 200 posts. Then they discussed different annotation results, analyzed the reasons, and resolved disagreements. This process takes five rounds, each with 200 labels, and they reached an agreement. 
Two authors independently label the 2,300 posts(kappa coefficient = 0.86, p < 0.01). After disagreement was solved, 29.6\% of the posts were emotional, and 70.4\% of them were informational. Because of the imbalance of the data, we oversampled the data, adjusted the ratio of an informational post to emotional post to 1:1, totaling 3000 posts as the dataset for modeling. The overall accuracy was 0.86, f1-score is 0.87/0.85(information/emotion).


\textit{Reply Generation Model}.
For 22,000 pairs of posts and replies from real human users. The data contain the post title, text, picture, topic ID, view times, reply times, reply user ID, reply content, and reply update time. Then we performed data cleaning and filtering. 
\begin{itemize}
    \item Type filtering. We filtered out information posts using our classification model.
    \item First reply. We only extract the first reply of each post, which is the most relevant reply to the content of the post because subsequent replies may be influenced by the previous replies. 
    \item Advertisement. The research team members checked all data manually for advertisements. Then we delete all advertised posts.
    \item Attack. We checked all posts manually. After discussion, removed all explicitly offensive replies.
\end{itemize}

After filtering, 81,000 post-reply pairs are left as data set. We trained our auto-reply robot using this data set.

\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/evulation_final.png}
  \caption{Comparison of human rating on four dimensions. t-test results are 1)On correct: 4.37 vs 4.52, {$p$} > 0.1; 2)On appropriateness: 3.38 vs 4.16, {$p$}<0.01; 3)On willing-to-reply: 3.23 vs 3.91, {$p$}<0.01; 4)On emotion support:3.28 vs 3.34, {$p$}<0.01.}~\label{fig:evaluation}
\end{figure}



\subsection{Chatbot Performance}
%\textcolor{red}{question:compare with retrieval, XiaoIce}
We use automatic evaluation and human evaluation to valuate our chatbot performance in comparison to actual human agents.

\subsubsection{Auto Metric}
BLEU     \cite{Papineni2002BLEU} is an automatic evaluation metric that is widely used in natural language generation. BLEU score represents the similarity between output response from agent and response from humans according to n-gram matches. BLEU has been extended to a dialogue model. We applied this metric to testing data sets containing 2,000 posts. The BLEU score is 0.23 which is moderate score(Xu et al. evaluated their model with score of 0.36 and 0.345.     \cite{DeepProbe,NewChatbot:Xu:2017:NCC:3025453.3025496})


\subsubsection{Human Evaluation}
Based on previous work and the singularity of this study, we identified four dimensions for the evaluation of responses to posts: 1) \textit{correctness}. The response should be grammatically correct and smooth. 2) \textit{appropriateness}. The reply should be relevant to the topic of the post    \cite{Ritter2011Data}. 3) willingness to reply. A response should motivate the post owner to reply and communicate more deeply. 4)emotional support. Pregnant women often use online discussion forums and social media to seek support    \cite{Invesgating:10.1145/3134685}.

We randomly selected 200 posts, each corresponding to an AI and human response, thus a total of 400 pairs of post-reply. We asked five participants (five participants are all graduate students major in computer science, aged: Mean 23.3 SD 0.84, three females two males )to rate each response according to the dimensions of correct, appropriate, willingness to reply and emotional support on a 5-point Likert Scale range from strongly disagree (-2) to strongly agree (+2). Intra-class correlation (ICC(3,1) have a range from 0.74 to 0.99. The quality of a reply is measured through the average value of participants' ratings.
We performed a t-test to examine the quality of the response type (chatbot, human) regarding the four dimensions (Figure \ref{fig:evaluation}). 



\begin{figure}[hptb]
  \centering
  \includegraphics[width=\textwidth]{figures/dialogue_example_finnal.png}
  \caption{ Example of post and chatbot's reply in Chinese(right) and English translation(left)}~\label{fig:dialogue_example}
\end{figure}


Although it does not perform as well as humans in four measure dimensions, to our knowledge, it is the only chatbot that can target the topic of pregnant women based on state-of-the-art AI model.


\subsubsection{Categories of Chatbot Replies}
Although chatbot's replies are based on the content of the post, their types are diverse. We categorize chatbot's replies according to the type of emotional support. Emotional support is described as the transmission of information about a person being cared for and loved in intimate situations involving mutual trust
    \cite{cobb1976social}. Previous works     \cite{yoo2014giving,greene2003handbook} have categorized the forms of emotional support or dialogue action. Yoo et al.    \cite{yoo2014giving} had categorized emotional support into four categories:(a)empathy/sympathy, (b)encouragement/reassurance, (c)care/physical affection, and (d)universality/interrelationship    \cite{yoo2014giving}. Greene and Burleson    \cite{greene2003handbook} concluded that helpful emotional support could be divided into:(a)expressing acknowledgment, comprehension, and understanding of the target's feelings and situation, (b)legitimizing the target's feelings or actions, (c)encouraging the target to talk about and elaborate on the problematic situation and his or her feelings    \cite{greene2003handbook}. In our work, chatbot never expresses universality/interrelationship but encourages hosts to give more details about their experiences. Based on previous studies and following our research, we classified chatbot's replies into six categories: empathy/sympathy, encouragement/reassurance, care/physical affection, bot self, question, and passing on luck.

\textbf{Empathy/Sympathy}. chatbot expresses empathy, sympathy, understanding, worry, regret    \cite{yoo2014giving}, or indicates that it has the same feelings or experiences with statements such as  \textit{I understand you very well, this process is very difficult}. It expresses the same feeling, e.g., \textit{Same feeling}. Simple expressions are also considered to belong to this category such as: \textit{How could it be so serious?}; \textit{Oh my god}; \textit{Why is that? I have never heard of that!}; \textit{This is too exaggerated!}

\textbf{Encouragement/Reassurance}. chatbot expresses hope, wishes, trust, congratulations, motivation and praise in using expressions such as: hang in there, stay strong, keep marching, do not give up    \cite{yoo2014giving} as well as:\textit{relax, take it easy}; \textit{hope everything goes well}; \textit{congratulations on your baby}; \textit{So cute}; \textit{Admire you}; \textit{Best wishes for you}.

\textbf{Care/Physical affection}. chatbot offers specific suggestions for expressing care such as:\textit{Take care of yourself}; \textit{go to bed on time}; \textit{drink more water}. Sending some simple emojis is also grouped into this category, such as: [hug hug hug]; [happy happy happy]. In other cases, chatbot seems to have no idea what to do. It replies:\textit{I do not know, I cannot do it, I also want to ask why, I do not know how to observe, can anyone help me?}.

\textbf{Botself}. chatbot sometimes acts like a real pregnant woman, describing her personal experiences and opinions, or praying for herself. For example, it described its life: \textit{ I am going to the hospital next week for a B-mode ultrasound; I like sweet food lot; my due date is 6.11; I dreamed about a snake last night}. It also expressed its own unique opinions, such as \textit{dreams are contrary to reality; the biological mother is the best; gender is not important, health is good}. Besides, chatbot sometimes prays for itself under other people's posts, such as \textit{Bodhisattva, please bless me}. Although its reply has nothing to do with the post's host, it would still be replied to by others with expressions such as \textit{Hope our wishes can be realized}. 

\textbf{Question}. chatbot asks questions of the host to give a more detailed description, such as \textit{What happened?}; \textit{When is your due date?}; \textit{What did your husband say?}. 

\textbf{Passing on luck}. 
There is a distinctive culture in the YOUBAOBAO community that is the transmission of good luck. When someone posts an announcement that she is pregnant or she will have a baby, other members like to reply: \textit{Pass on your good luck to me}. This sentence can also be used for other good things, such as giving birth to a boy. A pregnant woman who likes boys may reply: \textit{Pass on your boy's luck to me}. When a specific check-up goes smoothly, others will say: \textit{Pass me the good luck of your four-dimensional check-up}. Chatbot learned this ability and sometimes replied similarly.

==> old copies/4_study.tex <==
\section{The Explorative Study}
% \color{red}
% \begin{itemize}
%     \item overall intro
%     \begin{itemize}
%         \item RQ
%     \end{itemize}
%     \item study procedure
%     \begin{itemize}
%         \item experiment description
%         \item ethic
%     \end{itemize}
%     \item participants(community intro)
    
% \end{itemize}

% \color{black}

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{figures/procedure.jpg}
  \caption{Work flow of filed study. 1)Filter out informational-support-seeking posts. 2) Filter out posts who had been replied by human in 10 mins. 3) Randomly select posts to reply with a 50\% probability. 4)Human and auto script prevent negative replies generation.}~\label{fig:procedure}
\end{figure}


We aim to explore whether deploying chatbot as an active member in an online community for pregnant women would have an impact on the community building and individuals well-being. So a seven-days field study was conducted with aims of answering the following questions:
\begin{itemize}
    \item \textbf{Q1:} Whether the emergence of chatbot can increase the participation of community members?
    \item \textbf{Q2:} Can the reply of chatbot bring emotional support to the post owner?
    \item \textbf{Q3:} How do members of the community interact with the chatbot?
\end{itemize}


\subsection{Research Setting: Pregnant Women Online Community}
YOUBAOBAO is an online pregnancy community. The community provides a place for pregnant women to discuss a variety of topics, such as pregnancy, parenting, beauty, hospital. Each post is made under one of the topics. However, professional medical consultation is not to target user scenarios in this community. There are no professional doctors or third-party guidance professionals in this community.

User identities are divided into three categories: pregnancy preparation,  pregnancy period, and new mothers. All users are free to post. These posts can be viewed and replied on by any other users. Users can enter titles of up to 25 words or not enter a title, and input must not be less than six words and not more than 3000 words of text. When users are posting a post, the system will automatically select a topic according to the content. Users can also modify their post topic manually.


There are 164 topics in total in the YOUBAOBAO online pregnancy community. We collected half-year posts. According to statistical analysis, we found that this community produces about 100,000 posts per week with an average of 6 responses per post. However, about one-sixth of the posts did not receive replies.

We focus on five topics according to our research aim: Pregnancy preparation, The first trimester, the second trimester, the third trimester, and Newborn babies. Because our chatbot aims to provide support to pregnant women, we chose these five topics according to the pregnancy stages. Other topics are related to female topics, but the relationship with pregnant women is not very strong, such as clothing, skincare, jokes, and housework. In these five topic groups, 5,000 posts are generated per day.

\begin{figure}
\centering
  \includegraphics[width=0.9\columnwidth]{figures/screen.png}
  \caption{A screenshot of a post page from the YOUBAOBAO community }~\label{fig:forum_post}
\end{figure}




\subsection{Procedure}
We conducted a between-subjects field study at the post level. We do not want the early revealing/exposure of the bot's identity to influence our experiment results. As suggested by previous literature        \cite{luo2019machines,Recommend_comment_Morris2018TowardsAA,Jakesch:2019:ACP:3290605.3300469}that users do have biased perception on AI-generated contents. So we deployed the chatbot, which is framed as a human member in OHCs, to reply to emotion-seeking posts automatically.

The flow of the study is shown in Figure \ref{fig:procedure}. In order to balance the data volume of the two groups of control experiments, every new post that has not received a timely response within ten minutes will be randomly assigned to a group. In the experimental group, the post will be replied by the chatbot, and in the control group, it will not be replied by the chatbot.
In other words, all posts in the experimental group did not get a response within ten minutes, and these posts were judged to be an emotion-seeking post by the classification model.

To determine chatbot's response time, we collected posts for half a month; the total posts were 60,000 posts. We analyzed the time of the first replies for each post. As shown in Figure \ref{fig:replyTime}, the median time is ten minutes. 


In order to determine the study time and the time point of the experimental data collection, We collected the posts of one month. The time of penultimate reply of each post was selected as the last active time of the post. We found that the average active period of posts is six days. So we collect data on the seventh day after the study ends. 
Moreover, we get rid of all the replies after seven days of posting. The data were divided into two groups: the chatbot group(posts which were replied by chatbot) and the non-chatbot group(posts which were not involved by chatbot). 




\textbf{Extra Protection.}
We took precautions to conduct this study as ethically as possible. In preparing the corpus, we have filtered out aggressive words, negative words, or advertisements. In the deployment script, we added an automatic checking function to check if the content for output contains aggressive or negative keywords and. If the script detected exception, the chatbot would discard the replies to this post. During the experiment, our research team staff checked the posts in real-time and assessed whether there were any inappropriate or unintended attacks on others. Besides, after the experiment, we sent private messages to all members who interacted with our chatbot to inform them of chatbot true identity. %This project was approved by the Institutional Review Board. 

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{figures/time5.jpeg}
  \caption{Distribution of each post's first reply time }~\label{fig:replyTime}
\end{figure}





==> old copies/5_finding.tex <==
\section{Findings}
% We made quantitative and qualitative analysis of the behavior and content of the post's owner and other members. 
We explored whether deploying chatbot as active member in an online community for pregnant women would have an impact on the community building and individuals well-being. 

For community building, active participation from members in the community is the critical success factor for a sustainable community    \cite{Wagner2009Creating}. We measured the participation of all members according to the reply behavior of post owner after posting, and other members' reply behavior on posts, including unique participants, their reply times, sentence length, reply timeliness. 

For individuals' well-being, chatbot gives timely emotional support to the post owners of posts in the online pregnant women's community. We compared their emotional state in posting with that in chatbot's replies. 

According to our emotion/information classification model, there were 3694 non-informational posts without timely replies within the first 10 minutes during the seven days of the study. There were 1848 posts in the group with the chatbot; 120 of these were deleted by the post owner, leaving a remaining 1728. There were 1846 posts in the group without chatbot; 129 of these were deleted by the post owner, leaving 1717 posts. 


\input{5_finding1.tex}

\input{5_finding2.tex}

\input{5_finding3.tex}

\input{5_finding4.tex}

\input{5_finding5.tex}











==> old copies/5_finding1.tex <==
\subsection{Finding 1: Posts get faster replies after chatbot replied}
We analyzed the behavioral data of all members (not including post owner), as shown in Table \ref{tab:dynamic}. We compare the post dynamic and participation of members. We performed a t-test to examine the effect of the chatbot.

\textbf{Post}. As shown in Table \ref{tab:dynamic}. There are 1728 posts in the chatbot group, and the chatbot made the only reply in 789 of these posts. There are 1717 posts in the non-chatbot group, and 625 of these remained without replies. The chatbot group had fewer view times(average views times per post: 193 times vs 241 time, {$p$} > 0.05), but more people left replies(average reply times per post: 7.18 times vs 5.47 times, {$p$} > 0.05). There is no difference in post length(average length per post:91.75 words vs 91.15 words, {$p$} > 0.05). Although the number of unique participants in the chatbot group was higher(Average unique participants per post: 4.45 users vs. 3.38 users, {$p$} > 0.05 ), there was no significant difference between the two groups. Overall, the chatbot has no significant effect on the post.

\textbf{Members Participation}. As shown in Table \ref{tab:members}. There was no significant difference in the times of replies between the members not including owners in two groups, whether they reply to posts or to others(total reply times: 5.41 times vs. 6.3 times, {$p$} > 0.05; reply times to post: 3.53 times vs. 2.61 times, {$p$} > 0.05). However, there were significant differences in time. The average first reply time of each post is 12.7 minutes in the chatbot group and 254 minutes in the non-chatbot group. This result is because the first reply in the chatbot group was produced by the chatbot. Furthermore, the interval between the second reply time and the first reply time was significantly shorter in the chatbot group than in the non-chatbot group(Second replies gap time: 349 mins vs. 462 mins, {$p$} < 0.05). In order to confirm our conclusion more accurately, we calculated the time interval of the first five replies for each post. We found that the overall reply time of members was significantly faster in the chatbot group than in the non-chatbot group(average replies gap time: 441 mins vs. 607 mins, {$p$} < 0.01). 

In summary, there were no obvious advantages in the number of participants, but it significantly increased the speed of the reply of other members.


%life cycle

% Although people in the chatbot group participated more promptly, there is no significant difference between them in maintaining a post's life cycle (1100 vs 1067, P > 0.05). 


%Members of the chatbot group participated much earlier in time. But it has no effect on extending the life cycle of a post.
 %bot的快速留言，吸引了人们更提前的加入评论，但是对他们与其他成员的交流的积极性没有影响。对一个post的生命周期也没有影响。
%原因分析：bot的快速响应，吸引了更多人。但是并不是针对bot的回应，而是引起了她们的兴趣。那么对于主人来说，bot的内容让孕妇更开心了


\begin{table}
  \centering
  \begin{tabular}{p{100pt} | r r}
     \toprule
    & {\small {chatbot Group}}
      & {\small {Non-chatbot Group}}\\
    \midrule
    Total posts (count) &   1728    &   1717 \\
    View (times)  &   193(2465) &   241(3708) \\%P = 0.424
    Replies (times)   & 7.18(30)  & 5.47(30) \\ % p = 0.4
    Post length (words)    & 91.75(153) &   91.15(148) \\ %p = 0.487
   Participants(users)  &   4.45(15.9)    &   3.38(20.1) \\%0.76

    
     \bottomrule
 
  
   \end{tabular}
  \caption{Post dynamic in different dimensions between chatbot group and non-chatbot group. Asterisks represent pairwise significant differences, which are noted as:{$p$}<0.01(**) and {$p$}<0.05(*), numbers in parentheses represent standard deviation}~\label{tab:dynamic}
\end{table}




\begin{table}
  \centering
  \begin{tabular}{p{100pt} | r r}
     \toprule
    & {\small {chatbot Group}}
      & {\small {Non-chatbot Group}}\\
    \midrule
  
 Total replies (times)      &   5.41(26.2)    &   6.30(35.1)\\%0.305
         \hline
     Replies to post (times) &   3.53(11)    &   2.61(14)\\%p=0.787
       \hline
   % reply time per post(min)** & 1596(2992)  &   1896(3185) \\%p =0.000
    Second replies\\gap time (mins)*    &   349(1368) &   462(1725) \\%0.013
       \hline
    Average replies \\gap time (mins)**  &  441(1324)  & 607(1764)\\%0.001
     
     %关于other members的reply rate，因为本身就很低，大部分都是来自post owner的，所以这里计算all members reply rate没意义，并且，事实，两组比较没有差异
    %Reply rate on replies**     &      0.42(0.49)    & 0.39(0.48)\\%0.000
    %Other members reply rate on replies    & 0.04(0.2)   &   0.04(0.2)\\%0.827 
  \hline
     Reply length(words) &   17.42(14.2)   &   17.81(16.6)\\%0.073
   % Reply time(min)**     &   459(1262)    &  382(1059)     \\%0.002受到很多因素影响：人们看到post的时间；reply的时间分布很长，有些reply非常靠后；受到其他reply内容影响，与我们的bot无关
    % Reply rate on first reply     &   0.46(0.49)    &    0.55(0.49)   \\%0.558
    % Reply time on first reply &   286(1101)   &   375(1058)   \\%0.095  0.98都是主人回复的，这里讨论整体没意义

     
    
   \bottomrule
 
  
   \end{tabular}
  \caption{Members not including post owner behavior in different dimensions between chatbot group and non-chatbot group. Asterisks represent pairwise significant differences, which are noted as:{$p$}<0.01(**) and {$p$}<0.05(*), numbers in parentheses represent standard deviation}~\label{tab:members}
\end{table}






% \begin{figure}
% \centering
%   \includegraphics[width=0.9\columnwidth]{figures/replytime_COMPARE.png}
%   \caption{Comparison of replies and posting intervals between chatbot group and non-chatbot group in the each position of reply}~\label{fig:reply_time_compare}
% \end{figure}



==> old copies/5_finding2.tex <==
\subsection{Finding 2: Post owners are more active in communicating with others after chatbot replied} 


We analyzed the behavioral data of the post owner, as shown in Table \ref{tab:host}. We compared the two groups in post owner reply behavior. We performed a pair-wise t-test to investigate the effect of deploying a chatbot into the community.

\textit{Reply times} means the total times the post owner reply to other people after posting in each post. There was no significant difference between two groups(1.78 times vs 1.36 times, $p$ > 0.05).

\textit{Reply rate on replies to post}. This rate indicated the probability of a reply to the post being replied by the post owner. The average reply rate of each posts was higher in chatbot group than non-chatbot group(0.37 vs 0.34, {$p$} < 0.01).

\textit{Reply rate on the first replies}. This rate indicates the probability of the first reply to the post being replied by the post owner. The average reply rate of each posts was lower in chatbot group than non-chatbot group(0.44 vs 0.5, {$p$} < 0.01). In other words, chatbot got fewer post owner replies than the human who replied firstly to post in the non-chatbot group.

\textit{Reply gap time to the first replies}. This gap time indicates the interval between the post owner's first response behavior after receiving the first reply. The average gap time was faster in the chatbot group than the non-chatbot group(283 mins vs. 399 mins, {$p$} <0.05). 

\textit{First reply gap time}: This gap time indicates the interval between the post owner's first response behavior after posting. The average gap time was faster in the chatbot group than the non-chatbot group. It means post owner went back to post(replied to others) faster in chatbot group than non-chatbot group(450 mins vs. 727 mins, {$p$} <0.01). 


In summary, with a chatbot involved, the participation of post owners in posts has been significantly improved, which can be seen clearly from the reply number/rate to the reply time. We speculate that this is because chatbot has increased the activity of posts. However, in response to the first reply, the enthusiasm of post owners in responding to chatbot's replies is obviously lower than that of the real user, for which we will explain reasons later.






\begin{table}
  \centering
  \begin{tabular}{p{120pt} | r r}
     \toprule
    & {\small {chatbot Group}}
      & {\small {Non-chatbot Group}}\\
    \midrule

    %post owner
    Total replies (times) & 1.78(5.1)  & 1.36(4.9)  \\%0.096
    \hline
  Reply rate on replies to post(\%)**     &   37(48)    &  34(47)     \\%0.000
     \hline
  % post owner reply time** &   446(1203) & 363(974)\\%0.000
     Reply rate on the first replies (\%)**    &   44(49)    &   50(50)    \\%0.000
     \hline
   Reply gap time to the first replies (mins)*    &   283(1081) &   399(1096)\\%0.028
    \hline
    The first reply gap time(mins)**     &   450(1367)    &   727(1815)    \\%0.000
    \hline
    

    Reply length(words)  & 15.1(16.5)  &   15.76(16.4)   \\%0.499

 \bottomrule
 
  
  \end{tabular}
  \caption{Post owner behavior in different dimensions between chatbot group and non-chatbot group. Asterisks represent pairwise significant differences, which are noted as:{$p$}<0.01(**) and {$p$}<0.05(*), numbers in parentheses represent standard deviation}~\label{tab:host}
\end{table}



==> old copies/5_finding3.tex <==
\subsection{Finding 3: Chatbot inspires more emotion raise and less emotion drop}
In the evaluation of the chatbot, the emotional support score of the chatbot is significantly lower than that of humans. However, in Finding 2, we found that the chatbot group had higher post owner activeness. Contrary conclusions motivate us to analyze more: 1) Does chatbot's replies really have a positive impact on the post owner's emotions?; 2) Can the chatbot provide emotional support for the post owner?; 3) Does the timeliness of the chatbot's replies improve the effect of emotional support? 


We classify post owner replies into three categories according to emotional valence    \cite{lubis2015study}: positive(Happiness, Contentment), negative(Anger, Sadness), and neutral. Two annotators annotated each post and the post owner's replies emotional valence score(-1,0,1) to the first replies (kappa coefficient = 0.88) and annotated the chatbot's replies according to six categories (kappa coefficient = 0.84). Two annotators annotated the corpus and reached an agreement through discussion. In the chatbot group, 783 first replies were replied by post owners, while 536 replies in the non-chatbot group received replies from post owners. We classify emotional changes into three categories according to previous work    \cite{lubis2015study}: Emotional\_drop (from positive to negative, from neutral to negative, from positive to neutral), Emotional\_raise (from negative to positive, from negative to neutral, from neutral to positive), Emotional\_nochange (Emotions of the posts are consistent with the emotions of the reply).



As shown in Table \ref{tab:emotion_change}, the chatbot's replies can lead to more emotions\_raise, and emotions\_drop is lower here than in the case of replies from humans. We do not attribute emotional\_drop to negative effects because negative emotional expressions can also reduce stress    \cite{pennebaker2011expressive}. 

\textbf{Emotion\_drop}. We can divide the decline of emotional valance into three situations: 1) post owners share their negative emotions after getting the attention of others, such as \textit{post owner: I hope I can give birth as soon as possible; chatbot: take it easy; post owner: It is too difficult [cry][cry][cry].} 2) The post owners expressed their joy. Replies contained more inquiries and post owners gave a declarative response, such as \textit{post owner: It is gratifying to see a little change every day; chatbot: how many weeks have you had; post owner: fifteen weeks}.

\textbf{Emotion\_raise}. We can also divide the promotion of emotional valence into three situations: 1) post owners expressed some of their concerns, and, after replies comforted them, they showed reassurance, such as: \textit{post owner: Will the baby's legs turn into O-legs; chatbot: So do mine, which is very common; post owner: that's good.} 2) Encouragement in replies made post owners feel extremely friendly, such as \textit{post owner: I'm insomniac, and I still can't sleep at 3:00 in the morning; chatbot: Take a rest and don't get too tired; post owner: Wow!!! I want to hug you!} 3) post owner describes daily life, and the blessing in the replies makes them feel very happy, such as \textit{post owner: Go to the hospital tomorrow; chatbot: Everything will go smoothly; Ha! Thank you.}


% Emotion\_drop does not indicate something negative. Thus, we cannot analyze whether the chatbot or a human in the real community is the better active member based on the emotion\_change factor. However, there is a very serious problem with chatbot. It can only be identified in a situation as having a negative effect on the emotions of pregnant women, i.e making an irrelevant replies which would not occur in replies from humans. This may be one of the areas where our chatbot needs to be improved in the future. 

In summary, we found that the chatbot improves the emotional valence of pregnant women more than humans, decreases the emotional valence of pregnant women less than humans.







 
\begin{table}
\centering
\begin{tabular}{l |r r }
 \toprule
    {\small{Type}}
    & {\small {chatbot}}
    & {\small {Human}}\\
    \midrule
Emotion\_drop     & 14\%      & 18\%     \\
Emotion\_raise    & 48\%      & 38\%   \\
Emotion\_nochange & 38\%      & 44\%   \\
\bottomrule
\end{tabular}
\caption{post owner emotional change by chatbot and human reply(t-test: {$p$} = 0.178)}~\label{tab:emotion_change}%p=0.178
\end{table}



==> old copies/5_finding4.tex <==
\subsection{Finding 4: Chatbot encourages pregnant women to be more willing to communicate}

We collected the types of post owner replies. Through analysis, we found that several types often occur in the post owner replies to the chatbot: incomprehension, more communication, gratefulness, emotion disclosure, expressing a wish, agreement, asking for permission to following each other, and a simple emoji.

40\% of the post owner replies included more communication (The second highest type is gratefulness(13\%)). When the chatbot expresses Empathy/Sympathy, Care/Physical affection, Botself, and Question in its replies, the most frequent response from the post owner was more communication(not including in the case of "Passing on luck" and "Encouragement/Reassurance"). Pregnant women have a great desire to talk to other members    \cite{Romano2007A} even though the chatbot replied with simple words, such as:


\begin{itemize}

  \item Empathy/Sympathy
   
  \textit{chatbot: I know your feeling very well.}

            \textit{post owner: My husband and I are both at work. My family is always urging me. Do you think I am under too much mental pressure?}
            
    \item Care/physical affection
    
    \textit{chatbot: You'd better visit doctor.}

            \textit{post owner: Well, I'm going to check it tomorrow.}
 
    \item  Botself
    
    \textit{chatbot: I like eating eggs.}

            \textit{post owner: Ha! Now I do not dare eat too much every day.}
            
    \item  Question
    
    \textit{chatbot: What happened?}

            \textit{post owner: Can we follow each other? I will tell you the detail.}
\end{itemize}

13\% of the post owner replies included gratefulness, such as: \textit{Thanks, you too}. 12.7\% included emotional disclosure, such as: \textit{Expectation and nervousness; I feel too painful}. 7.5\% included expressing wish, such as: \textit{Best wish for you; Hope everything will go well with you too}. 6.9\% included post owner's interest in chatbot, such as: \textit{When is your due?}.




\begin{table}
  \centering
  \begin{tabular}{ p{120pt} | p{40pt} | l  r}
     \toprule
    {\small{chatbot reply to post}}
    & {\small {Reply rate}}
    & {\small {post owner reply to chatbot}}
    & {\small {ratio(\%)}}\\
    \midrule
 
    \multirow{3}{*}{Empathy/Sympathy} &   \multirow{3}{*}{49.95 }   &   More communication &   33.3 \\
    & & Interest in chatbot   &   29.7 \\
    &   &   Emotional disclosure   &   27.8 \\
    
    \hline
     
     
    \multirow{3}{*}{Encouragement/Reassurance} &   \multirow{3}{*}{42.7 }   &   Gratefulness &  33.7 \\
    &   &   More communication  &   29.2 \\
    &   &    Emotional disclosure  &  24.7 \\
    
    \hline
    
    \multirow{3}{*}{Care/Physical affection} &   \multirow{3}{*}{60.61 }   &   More communication &   72.4 \\
    & & Agreement   &   11.7 \\
    &   &   Emotional disclosure  &   10.3 \\
    
    \hline
    
    \multirow{3}{*}{Botself} &   \multirow{3}{*}{44.6 }    &   More communication  &   62.7 \\
    &   &    Interest in chatbot &   19.7\\
    &   &     Emotional disclosure  &  17.6\\
     
    \hline
   
    Passing on luck &   42.37   &   Expressing wish  &   100 \\
    
    \hline
    
    
    \multirow{3}{*}{Question} &   \multirow{3}{*}{66.22 }   &   More communication &   83.1 \\
    &   &    Incomprehension  &   11.8 \\
    &   &  Emotional disclosure  &   5.2 \\
     

  
     \bottomrule
  \end{tabular}
  \caption{chatbot's replies to posts and post owners' replies to chatbot}~\label{tab:reply_reply_map}
\end{table}
% %多表达同理心，更能激发用户的自我曝露，适当的让bot有自己的个性，故事，可以吸引他人的兴趣



==> old copies/5_finding5.tex <==
\subsection{Finding 5: Chatbot triggers pregnant women emotional disclosure}

12.7\% post owner replies included emotional disclosure. As shown in Table \ref{tab:reply_reply_map}, chatbot's each emotional support type (not including "passing on luck") was able to trigger post owner emotional disclosure. When chatbot provided the two emotional support(empathy/sympathy and encouragement/reassurance), post owners replied emotional disclosure more than providing other emotional support types(empathy/sympathy:27.8\%, encouragement/reassurance:24.7\%, care/physical affection:10.3\%, botself: 17.6\%, question: 5.2\%).

\begin{itemize}

  \item Empathy/Sympathy
   
  \textit{chatbot:Women are too difficult.}

            \textit{post owner:Being women is so tired.}
            
    \item  Encouragement/Reassurance
    
    \textit{chatbot:Do not mind, take it easy. }

            \textit{post owner: I became fragile after having a baby. [cry]}
            
    \item Care/physical affection
    
    \textit{chatbot: Pay attention to rest}

            \textit{post owner: OK! I only hope my baby is healthy.}
 
    \item  Botself
    
    \textit{chatbot: I have not been to the hospital yet}

            \textit{post owner: All mothers are so tired. [cry]}
            
    \item  Question
    
    \textit{chatbot: What happened?}

            \textit{post owner: Can we follow each other? I will tell you the detail.}
            
\end{itemize}

==> old copies/6_discussion.tex <==
%关于身份disclourse后的user的interview-反应
\section{discussion}
% \textcolor{red}{future human in the loop design,chatbot low reply rate,more active,appearance is a kind of support(late-night)}

% \pzh{Our study shows that conversational agents can be useful in synchronous online health communities.}
% Conversational agents can be useful in synchronous conversational settings, as illustrated in study. 
Women are at high risk of mental illness during the pregnancy period and online health communities (OHCs) can provide valuable emotional support to pregnant women. 
\pzh{Our study shows that the intervention of our chatbot's response not only motivates other community members to reply to the original posters (OPs) more quickly but also boosts the OPs to reply to their supporters.}
% In this work, the results show that while controlling other factors, the intervention of chatbot's response motivated other community members to reply to the original post quicker; the original poster, also the emotional-support-seeker, is more active in replying to other community members.

However, little is known about how members of the community interact with anonymous chatbots. How do people respond to chatbot? What are the advantages and disadvantages of chatbot compared to humans? We propose some possible reasons for some findings and discuss several additional themes that emerged from our findings.




\subsection{More Active Behavior}

Finding 1 shows that chatbot's replies improve the overall reply speed of posts. To explain this phenomenon, we speculate that this may be partially due to chatbot's timely replies. When people view a post that has been replied, as a non-first reply person, the behavior of the reply seems to be less critical and more comfortable to produce. \pzh{ Also, the content of chatbot's replies could provide other members more thoughts     \cite{zhenhui2020chi}.} They may choose to reply directly to the chatbot or the post again.
%related to the community's display mechanism. Under each topic, there are three different ways to display posts: the default, the essence, and the latest. Posts are presented in a list. The default display is based on-time ordering and adds the factor of hotness. A post that has just gone up will likely not appear in the default list if it has not yet received any replies. However, if it has been replied on, it will immediately appear at the top of the default list. Furthermore, even if it was posted ten minutes ago, it will still appear before a new post that was posted one minute ago.

% post owners (be consistent)
Finding 2 shows that original posters are more active in replying to others. We suspect that this is perhaps due to the chatbot's timelier reply time. After posting, the post owners usually look forward to receiving a reply. This hopeful expectation gradually decreases as the waiting time increases. If a post owner receives a positive encouragement after a short period, then her enthusiasm for being active increases, and the interaction behavior thereby increases
in volume and speed. 


\subsection{Lower Reply Rate than Human}
Although the chatbot can offer pregnant women emotional support, the data analysis shows that chatbot's reply rate is significantly lower than that of humans, as shown in Table \ref{tab:dynamic}(Reply rate:0.44 vs. 0.5, {$p$} < 0.01). We wanted to learn why chatbot's replies get lower reply rates than humans.


We analyzed what the advantages of human replies and chatbot replies characteristic are. Besides, we analyzed the reason that other members replied to the chatbot. We hope to provide a reference for future emotional support chatbot in OHC design by learning the advantages of human replies and enhancing chatbot's replies characteristics.


\subsubsection{Human Replies}

The types of human replies are similar to  the chatbot, but they have some features that chatbot does not currently have:

\begin{itemize}
    \item Specific professional information.
    
    
    Although the post owner is encouraged by both the chatbot and humans, the human replies often contain some professional information, such as: \textit{The examination index is not more than 10,000, do not worry}.
    
    \item  Understanding the picture.
    
    The chatbot cannot understand the picture. Many of the human replies include the replies on the content of the picture posted, such as: \textit{The baby's hair is beautiful, which barbershop did you go?}
\end{itemize}

\subsubsection{Chatbot Replies}

Previous study     \cite{Care_for_bot_Lee:2019:CVC:3290605.3300932} have demonstrated that caring for a chatbot can help people gain greater self-compassion than being cared for by a chatbot. We also experience this phenomenon in our study. There is a distinctive culture in the YOUBAOBAO community. We call it "Good Luck Delivery." when someone would post that she is pregnant, had a successful delivery, had a boy or girl or have twins or something similar or even report that the results of the examination are perfect, someone will reply below: \textit{Pass on the good luck of the girl / Pass on the good luck of the examination / Pass on the good luck of the pregnancy}. Our chatbot learned this behavior. When the chatbot express that it also would like to have good luck, 42.37\% of the post owners replied. The post owners sent their blessings to the chatbot. However, if the chatbot's replies were only for blessings, i.e., "pray" rather than using a specific "pass on" expression, the reply rate would only be 9.26\% \textit{e.g. I hope your wishes will be realized}. 

The chatbot sometimes does not express care, encouragement, or empathy directly but describes its own life or expresses some opinions, not specific to a post owner.
For example, \textit{chatbot: I would like to go to the hospital for my postnatal confinement; chatbot: I had a nightmare yesterday, and I woke up scared}. The post owner expresses their interest in the chatbot (The reply rate was 44.6\%): \textit{post owner: When is your postnatal confinement? post owner: What did you dream that was so scary?} Besides, when the chatbot replies \textit{Me too} or \textit{I feel the same as you}, and so on, people are also interested in the chatbot.  Because they think they have found someone similar to themselves. For example, there was the post: \textit{Frequent urination at night slept poorly}. The chatbot replied: \textit{Me too}. The human reply was: \textit{How many months have you been pregnant? Let us follow each other}. 
%未来的bot可以有自己的个性，表达自我，提高互动性


If chatbot replied, "I do not know" or asked if someone else can help, it could seem useless, but most people thank the chatbot and express their feelings to the chatbot. It seems that when someone replies on it, it means that person was concerned, and that has already been a comfort.%\textcolor{red}{add interview as evidence}



\subsubsection{Other Members Replies to Chatbot}%简单谈谈，为什么会提高其他人积极性，哪些因素吸引了他们
%others reply bot
There were 29 posts with the chatbot's replies in which members other than post's post owner participated. The maximum number of rounds in the dialogues reached ten rounds. We categorized the reason that other members replied to chatbot:
\begin{itemize}
    \item Join the discussion and express one's personal situation.
    
    \textit{Other member: In my case, the doctor helped me listen to the fetal heart, but I could not hear it, but the B-scan showed that it could be heard.}
    
    \item Supplementary chatbot's reply
    
    \textit{chatbot reply: Drink more brown sugar water}
    
    \textit{post owner: Should I drink it or a child?}
    
    \textit{Other member: She meant, of course, that you should drink more brown sugar water. How could a child drink it?}
    
    \item Pass on the good luck from chatbot
    
    \textit{chatbot reply: I am about to have a baby, too.}
    
    \textit{Other member: Pass on your good luck.}
    
    \item Reply showing interest in chatbot and asking chatbot more
    
    \textit{Post: Never get pregnant before marriage. If you want to have an abortion, you should do it as soon as possible. Do not induce labor for six months like me. It is excruciating.}
    
    \textit{chatbot reply: I want to do it, too.}
    
    \textit{Other member: How many months have you been pregnant? What is the specific situation? If it is just a fight, it is better not to do it.}
    
    \item Emphasize the post owner's Intention
    
    \textit{chatbot reply: I do not know, either}
    
    \textit{Other member: She must have inflammation, or she will not have a recurring fever.}
    
\end{itemize}


% chatbot 注意时态和首字母大小写
\subsection{\pzh{Chatbot} for Late-Night Posts}
During our research, we unexpectedly discovered that \pzh{the} automated chatbot \pzh{has an advantage over humans -- it can provide timely replies for the posts created by insomniacs at late night.} 
% a unique advantage over humans. The chatbot provides timely replies for posts posted late at night by insomniacs. 
We collected all posts from 0 p.m. to 5 a.m. 30\% chatbot replies got replies from post owner. 38\% of post owners replied with emotional disclosure. 18\% replied with gratefulness. 

Furthermore, we selected posts that contained insomnia keyword, such as ``insomnia'', ``can not sleep'' and ``wake up again''. 4\% of the late-night posts explicitly express insomnia problems. 50\% of them received only chatbot's reply. 57\% post owners of these posts replied chatbot. Replies include complaints about insomnia, gratefulness, and negative emotions. 

% to target
In future work, researchers can consider using the chatbot, specifically \pzh{for} people who have insomnia at night. This auto-reply chatbot may solve the problem of people not receiving timely responses at night.
 
 
% \subsubsection{chatbot's Fans}

% chatbot got 21 notes of praise and had 19 fans. We carefully viewed the home page of each account trying to find out why they followed the chatbot. This confirmed that 7 users had abnormal accounts (i.e. blocked). There were 10 users on whose posts chatbot replied once (We could not determine if they had seen the chatbot in other posts). For five of ten users, the chatbot had posted the only reply on their post. Human member did not reply on them. Nine of ten users replied to the chatbot's replies. Their reply content includes: thanks, a request to follow each other, emotional disclosure.

% \subsection{State of post owners}

% We compared two situations: no replies, only chatbot replies. We found that pregnant women who received support
% were more involved in the subsequent community activity than those who did not. 
% In the non-chatbot group, 625 posts did not receive any replies in one week, and, after three weeks, 34 users deleted their non-replied posts. 16 people (2.7\%) deleted all their posts. At the time of our last data collection, one month after the experiment, 238 people had not posted again. 
% In the chatbot group, 763 posts received only chatbot replies in one week, and, after three weeks, 27 users deleted their non-replied posts. No one deleted all their posts here. One month after the experiment, 307 people did not post again. In the future, if a community employs a chatbot, guaranteeing that there will be no non-replied posts, the loss of participants may be greatly reduced.


% \subsection{Design Implications}

% Based on the findings in this study, we summarized following implications and takeaways that could be helpful for deploying chatbot as active member to an online community for pregnant women: 

% 1. Posts get faster replies and post owner are more active in communicating with others after chatbot replied (Finding 1 and Finding 2). To increase community participation, Designer can consider deploying a chatbot that provide timely reply in online community.

% 2. chatbot inspires post post owner more emotion raise and less emotion drop (Finding 3) and triggers post owner more communication desire (Finding 4) and emotional disclosure (Finding 5). Chatbot can benefit individuals in the community. This approach can be considered in a wider area, providing timely support to people in need of emotional support in the community, such as cancer community, breast cancer community, depression community.






% \subsection{members' perception}

% --------interview-----------

% -follower 10 people; positive response 20 people;  negative or normal response 10 people; no reply 10 people;21 like people

% -explain

% -question 1:evaluate response---do you like(1-5);do you trust(1-5);your emotional response;emotion support(1-5)

% -question 2:why you reply the bot? why you follow the bot? why you do not reply the bot?

% -question 3:Have you ever thought of it as a robot?

% -question 4:what do you want it do if you have a perfect AI bot,if you can trust it completely

% -question 5: can you accept a bot in the community? Is it need to disclose AI's identify? what do you think it can bring for you?

% -question 6: any question?

% -best wish for you.

% --------interview-----------


%\subsection{Bot Effectiveness }








==> old copies/7_future_conclusion.tex <==
\section{Limitation}
%culture human-in-the-loop identi
We acknowledge several important limitations to our work that
limit the design of field study.

As suggested by previous literature    \cite{luo2019machines,Recommend_comment_Morris2018TowardsAA,Jakesch:2019:ACP:3290605.3300469}that users do have biased perception on AI-generated contents. In order to avoid the influence of identity factors on the experimental results, we concealed the identity of chatbot from users before the experiment. We have adopted manual monitoring to ensure safety during the experiment. This human-in-the-loop approach is not good for the convenience of the design of automatic reply robots in future communities. How to automate the supervision will be an interesting future study. We exposed our true identity to users after the experiment, but we did not conduct post-experiment interviews with them. It may be better to include subjective factors in the analysis.

The community we choose is for one country. The pregnant women in the community use the oriental education background and live in the society of oriental culture. This limitation may bias the study results.


\section{conclusion}

We built a generative chatbot as active member in an online community for pregnant women. Results from a 7-days between-subjects field study show that chatbot's replies improve the participation activeness of members. Hosts are more active in replying to others and replying to chatbot with emotional disclosure and more emotion raise. Furthermore, we analyzed which type of replies can attract others.

In our study, the identity of the chatbot is anonymous. In the
future, we will explore the impact of identity on people's trust in OHCs. Moreover, we will improve chatbot's performance in understanding pictures, having specific personal identity (e.g.  "26-year-old, a new mother to a 2-month-old baby." in chatbot's homepage) and supporting multi-rounds dialogue.


%bot的error，文不对题
%根据post生成对应的comment，comment的type分布我们不可控，导致有些type的数量少，那么对应的reply的分析不一定准确，具有偶然性
%bot的个人信息不确定，有时候是备孕的身份，有时候是宝妈，以后可以做多个身份的
%没有图片信息


%以后可以公布身份，两种对比
%以后做特定个人信息的账号bot
%future 让对话更持久，多轮
%降低了其他人的参与度

